High-Dimensional Uncertainty Quantification via Active and Rank-Adaptive Tensor Regression

Uncertainty quantification based on stochastic spectral methods suffers from the curse of dimensionality. This issue was mitigated recently by low-rank tensor methods. However, there exist two fundamental challenges in low-rank tensor-based uncertainty quantification: how to automatically determine the tensor rank and how to pick the simulation samples. This paper proposes a novel tensor regression method to address these two challenges. Our method uses an $\ell_{q}/ \ell_{2}$-norm regularization to determine the tensor rank and an estimated Voronoi diagram to pick informative samples for simulation. The proposed framework is verified by a 19-dim phonics bandpass filter and a 57-dim CMOS ring oscillator, capturing the high-dimensional uncertainty well with only 90 and 290 samples respectively.

==> EPEPS'20_Tensor_Regression_for_UQ/conclusion.tex <==
\section{Conclusion}
This paper has proposed a tensor regression framework for high-dimensional uncertainty quantification. Our method has addressed two fundamental challenges: automatic tensor rank determination and adaptive sampling. 
%Our method is verified by a 19-dim phonics bandpass filter and a 57-dim CMOS ring oscillator. 
The numerical result has demonstrated the excellent capability of automatic rank determination of our method, and the simulation cost reduction by our adaptive sampling method.

% \section*{Acknowledgment}
% This work was supported by NSF CCF No. 1763699 and NSF CAREER Award No. 1846476.


==> EPEPS'20_Tensor_Regression_for_UQ/introduction.tex <==
\section{Introduction}\label{sec:introduction}
Fabrication process variations are a major concern in nano-scale chip design. To estimate and quantify the uncertainties caused by process variations, Monte Carlo (MC) is the mainstream uncertainty quantification (UQ) tool used in commercial EDA tools, but it requires a huge amount of simulation samples. Instead, stochastic spectral methods based on generalized polynomial chaos (gPC)~\cite{xiu2010numerical} offer an efficient alternative by approximating a stochastic circuit performance metric as a linear combination of some basis functions~\cite{zhang2013stochastic,He2019,ginste2012stochastic}. However, stochastic spectral methods suffer from the curse of dimensionality: a huge amount of simulation samples are required when the number of random parameters is large. 

Low-rank tensor methods are a promising technique to solve high-dimensional UQ problems~\cite{konakli2016polynomial,zhang2014enabling, zhang2016big,chevreuil2015least}. In~\cite{zhang2014enabling}, a high-dimensional gPC expansion is obtained via a low-rank tensor recovery, which estimates massive unknown output samples from a few simulation results. However, the method~\cite{zhang2014enabling} uses a fixed tensor rank, which is hard to estimate {\it a-priori} in practice. The most recent work~\cite{shi2019meta} uses a greedy rank-1 update until a good accuracy is reached. However, greedy rank-1 tensor update does not provide optimal solutions and can cause over fitting. Besides, it is not clear how to adaptively pick the simulation samples to reduce the computation budget.

{\bf Contributions.} This paper proposes a novel high-dimensional UQ solver based on tensor regression. 
In order to automatically determine the tensor rank, we employ a group-sparsity regularization in the training process.  %The regression model is solved via an alternating algorithm with an analytical solution in each sub-problem. 
We also develop an adaptive sampling strategy to reduce the simulation cost. This method balances exploration and exploitation of our model. Our method is used to quantify the uncertainties of a 19-dim phonic IC and a 57-dim electronic IC with 90 and 290 simulation samples respectively. 



==> EPEPS'20_Tensor_Regression_for_UQ/motivation.tex <==
\section{Motivation}
\label{sec:motivation}


==> EPEPS'20_Tensor_Regression_for_UQ/numerical_result.tex <==
\section{Numerical Experiment}
\label{sec:numerical_results}
We verify our algorithm by a photonic band-pass filter and a CMOS ring oscillator as shown in Fig.~\ref{fig:PIC_CMOS}. 
% \textbf{Synthetic function:} We first demonstrate our framework on Friedman1 dataset, which is a 5-dim nonlinear function:
% \begin{equation}
%     y(\vecpar) = 10\sin(10\parm_1 \parm_2)+20(\parm_3-\frac{1}{2})^2 + 10\parm_4 + 5\parm_5
% \end{equation}
% All the variables are uniform on $\left[ 0,1 \right]$. 
\begin{figure}[t]
    \centering
    \includegraphics[scale=0.3]{Figure/PIC_CMOS.png}
    \caption{Left: a photonic band-pass filter with 9 micro-ring resonators. Right: Schematic of a CMOS ring oscillator.}
    \label{fig:PIC_CMOS}
\end{figure}

\textbf{Photonic band-pass filter:} This benchmark has 19 Gaussian random parameters describing the variations of the effective phase index ($n_\text{neff}$) of each ring, and the gap ($g$) between adjacent rings and between the end ring and the bus waveguides. 
We set the highest polynomial order $p=2$ for each dimension, and initialize $\ten{X}$ as rank-4, and use $q=0.5$ in the regularizer. 
We initialize 60 samples with a standard LH experimental design, and further select 6 batches with 60 additional samples. The proposed tensor regression framework is compared with a fixed rank method, a random and an adaptive exploration sampling method (shown in Fig.~\ref{fig:pic19}).
%The adaptive sampling strategy slightly outperforms random sampling when the sample size is small. They are both better than a fixed-rank tensor regression.
\begin{figure}[t]
    \centering
    %\flushleft
    \includegraphics[width=1\columnwidth]{Figure/fig_19.eps}
    \caption{Result of the photonic filter. (a) Testing error on $10^5$ MC samples, achieving 98.3\% accuracy. (b) The estimated tensor ranks.}
    \label{fig:pic19}
\end{figure}

\textbf{CMOS ring oscillator:} This circuit has 57 Gaussian random parameters describing the variations of threshold voltages, gate-oxide thickness, and effective gate length/width. 
The simulation results are obtained by calling a periodic steady-state simulator repeatedly.
We set basis as order-2 in each dimension, initialize $\ten{X}$ as rank-5, and use $q=0.5$ in the regularizer.
We start from 140 standard LH samples, and adaptively select additional 7 batches with 210 samples. 
%Our method reduces the estimated tensor rank to 2. 
The results and comparison are summarized in Fig.~\ref{fig:adp57} and Table~\ref{tab:ring57}. 
%The adaptive sampling outperforms random sampling in terms of accuracy. 
%Table~\ref{tab:ring57} shows that the tensor regression framework outperforms the polynomial chaos expansion model with a standard total degree scheme.
%It achieves the 99\% approximation accuracy to $10^5$ MC samples with only 350 simulation samples. 

\begin{figure}[t]
    \centering
    %\includegraphics[width=3.3in]{Figure/adaptive57.eps}
    \includegraphics[width=1\columnwidth]{Figure/fig_57.eps}
    \caption{Results of the CMOS ring oscillator. (a) Testing error on $10^5$ MC samples (b) Probability density functions of the oscillator frequency.}
    \label{fig:adp57}
\end{figure}

\begin{table}[t]
\centering
\caption{Comparison with the gPC model with a total degree scheme.}
\label{tab:ring57}
\begin{tabular}{ccccc}
\toprule
& Proposed  & Total-degree gPC  & MC \\
\midrule
\# of variables & 855     & 1711         &  N/A      \\
\# of samples   & 290       & 1711         &  $10^5$   \\
    Mean        & 106.28  & 106.58    &  106.53 \\
  Stdvar        & 4.616     & 6.810      &  4.641     \\
   Error        & 1\%       & 4.84\%        &  N/A      \\
\bottomrule
\end{tabular}
\vspace{-10pt}
\end{table}

==> EPEPS'20_Tensor_Regression_for_UQ/preliminary.tex <==
\section{Background}
\label{sec:preliminaries}
%\subsection{Tensor Notation}
%Tensor representation of the the proposed 

%\zz{A lot of materials in this section are useless: you don't need to explain the total degree since you are not using it. Instead, you should give some background about tensors: a lot of people in this community do not know tensors and you will use it in your approach. The key is to only provide background materials that you will use. Please check the background section of my SPI 2016 paper.}
%\subsection{generalized Polynomial Chaos Expansion}
{\bf Generalized Polynomial Chaos.} Let $\vecpar = \left[\parm_1,\ldots,\parm_d \right] \in \R^d$ be a random vector describing process variations. We aim to estimate the interested performance metric $y(\vecpar)$ (e.g., chip frequency or power) under such uncertainty.
% %finite variance
% Consider a simple one-dimensional case firstly, generalized Polynomial Chaos (gPC) expansion approximates $y(\parm)$ as follows:
% \begin{equation}
% \label{eq:Unit_expansion}
%     y(\parm)\approx \hat{y}^{gPC}(\parm) = \sum_{i=0}^p {c}_{i}\uniGPC_{i}(\parm),
% \end{equation}
% where $\{\uniGPC_{i}\}_{i=0}^p$ are orthogonal basis functions up to polynomial order $p$, and $\{\vect{c}_{i}\}_{i=0}^p$ are their corresponding coefficients.
A truncated gPC expansion approximates $y(\parm)$ as
\begin{equation}
\label{eq:Multi_expansion}
    y(\vecpar)\approx \hat{y}(\vecpar) = \sum_{\basisInd \in \Theta} {c}_{\basisInd}\multiGPC_{\basisInd}(\vecpar),
    %=\sum_{|\basisInd|=0}^p \mat{c}_{\basisInd}\multiGPC_{\basisInd}(\vecpar),
\end{equation}
where $\basisInd$ is an index vector, and $\multiGPC_{\basisInd}$ is a polynomial basis function of degree $|\basisInd|=\alpha_1 + \alpha_2+ \cdots +\alpha_d$. If the joint probability density function of $\vecpar$ is $\rho(\vecpar)$, then the basis functions satisfy the orthornormal condition:
\begin{equation}
    \langle \multiGPC_{\basisInd}(\vecpar), \multiGPC_{\boldsymbol{\beta}}(\vecpar) \rangle= \int \limits_{\mathbb{R}^d} \multiGPC_{\basisInd}(\vecpar) \multiGPC_{\boldsymbol{\beta}}(\vecpar) \rho(\vecpar)d \vecpar=\delta_{\basisInd,\boldsymbol{\beta}}.
\end{equation}
Once the index set $\Theta$ is chosen, we need to determine the unknown coefficient $c_{\basisInd}$ for each $\basisInd \in \Theta$. The gPC only requires a small number of basis functions and simulation samples when the parameter dimensionality $d$ is small. However, a huge number of basis functions and simulation samples are required when $d$ is large. For instance, in the classical stochastic collocation method~\cite{xiu2010numerical}, the  number of simulation samples required to obtain $c_{\basisInd}$'s is an exponential or polynomial function of $d$.
%One of the most commonly used truncation scheme is the total degree one, which selects multivariate polynomials up to a total degree $p$, 
%\ie~$\A = \{ \basisInd | \vect{\alpha}_k \in \N, 0 \le \sum_\limit{i=1}^d \vect{\alpha}_i \le p \},$
%leading to a total of $K = \dbinom{d+p}{p}$ terms of expansion.


%With regard to estimating the corresponding coefficients, several popular methods include intrusive methods like stochastic Galerkin, and non-intrusive methods like pseudo-projection based stochastic collocation and regression-based stochastic collocation. Here we briefly introduce the regression method as follow: we view the true performance metric $Y$ as the summation of gPC expansion and a residual. Given some sample pairs $\{\vecpar_i, y(\vecpar_i)\}_{i=1}^N$, suppose under a total degree truncation scheme, we minimize the square error of the residual to solve coefficients $\vect{c}$:

% The coefficients can be estimated via a regression framework: 
% %we view the true performance metric $Y$ as the summation of gPC expansion and a residual. 
% given some sample pairs $\{\vecpar_i, y(\vecpar_i)\}_{i=1}^N$, we minimize the square error of the residual to solve coefficients $\vect{c}$: 
% \begin{equation}
% \label{eq:classical_ls}
%     \vect{c} & = \argmin_\limit{\vect{\hat{c}}} \| \vect{y}^T - \sum_{i = 1}^K {\hat{c}}_{i}\mat{\multiGPC}_{i} \|^2_2 = (\mat{\multiGPC}^T\mat{\multiGPC})^{-1} \mat{\multiGPC}^T \vect{y},
% \end{equation}
% where $\mat{\multiGPC} = \{ {\multiGPC}_{ij} = \multiGPC_j(\vecpar_i), i=1,\ldots,N, j=1,\ldots,K \}$.

% Although gPC expansion offers a good surrogate for the metric $y(\vecpar)$, it suffers the well-known curse of dimensionality. 
% The number of needed samples is linear on the unknown variables, $\frac{\left(d+p\right)!}{d!p!}$, which grows exponentially and quickly becomes unaffordable since simulations are usually expensive in real circuit simulators. 

{\bf Tensors.} A promising tool to overcome the curse of dimensionality is the tensor. A $d$-dim tensor $\ten{X} \in \R^{n_1 \times \cdots n_d}$ represents a $d$-dimensional data array, and it becomes a matrix when $d=2$. The $(i_1,\cdots, i_d)$-th element of $\ten{X}$ can be denoted as $x_{i_1 \cdots i_d}$. Given two tensors $\ten{X}$ and $\ten{Y}$ of the same size, their inner product is defined as:
\begin{equation}\label{eq:inner_pro}
    \langle \ten{X}, \ten{Y} \rangle := \sum_{i_1\cdots i_d} x_{i_1\cdots i_d} y_{i_1\cdots i_d}.
\end{equation}
A $d$-dim rank-$R$ tensor can be written as the sum of $R$ rank-1 tensors, known as a CP decomposition:
\begin{equation}
\label{eq:CP}
    \ten{X}=\sum_{r=1}^R \mat{u}_r^{(1)} \circ \mat{u}_r^{(2)} \cdots \circ \mat{u}_r^{(d)} = [\![\mat{U}^{(1)}, \mat{U}^{(2)}, \ldots, \mat{U}^{(d)}]\!],
\end{equation}
where $\circ $ denotes an outer product. The last term is the Krusal form, where factor matrix $\mat{U}^{(k)} = \left[\mat{u}_1^{(k)}, \ldots, \mat{u}_R^{(k)} \right] \in \mathbb{R}^{n_k \times R}$ includes all vectors associated with the $k$-th dimension. 
%For more details related to tensors, we refer readers to~\cite{kolda2009tensor}.

%The numer of unknown variables in Eq.~\reff{eq:classical_ls} is $K = \dbinom{d+p}{p}$, which grows exponentially in dimensionality. In regression schemes, , which quickly becomes unaffordable since simulations are usually expensive in real circuit simulators. 

%\subsection{Moment information in low-rank structure}

==> EPEPS'20_Tensor_Regression_for_UQ/proposed_method.tex <==
\section{Proposed Tensor Regression Method}
\label{sec:proposed_method}

\subsection{Tensor Regression Formulation}
We choose the following index set for the gPC expansion:
\begin{equation}
\label{eq:indesSet}
    \Theta=\left\{ \basisInd=[\alpha_1, \alpha_2, \cdots, \alpha_d]\; |\; 0\leq \{\alpha_i\}_{i=1}^{d} \leq p \right\}.
\end{equation}
This specifies a gPC expansion with $(p+1)^d$ basis functions. Let $i_k=\alpha_k+1$, then we can define two $d$-dimensional tensors $\ten{X}$ and $\ten{B}(\vecpar)$ with their $(i_1, i_2, \cdots i_d)$-th element specified as
\begin{align}
\label{eq:tensorDef}
x_{i_1 i_2 \cdots i_d}=c_{\basisInd} \; {\text{and}}\; b_{i_1 i_2 \cdots i_d}(\vecpar)=\multiGPC_{\basisInd}(\vecpar).
\end{align}

Combining \eqref{eq:Multi_expansion}, \eqref{eq:indesSet} and \eqref{eq:tensorDef}, the truncated gPC expansion can be written as a tensor regression model
\begin{equation}
   y(\vecpar) \approx \hat{y}(\vecpar) = \langle \ten{X}, \ten{B}(\vecpar) \rangle.
\end{equation}
It is worth noting that tensor $\ten{B}(\vecpar)$ depends on $\vecpar$. When the random parameters $\vecpar$ are mutually independent, $\multiGPC_{\basisInd}(\vecpar)$ can be written as the product of $d$ uni-variable basis functions for each parameter $\xi_k$. In this case $\ten{B}(\vecpar) $ is a rank-1 tensor.

Our goal is to compute $\ten{X}$ given a set of data samples $\left \{\vecpar_n, y(\vecpar_n)\right \}_{n=1}^N$. Assume that $\ten{X}$ has the rank-$R$ decomposition in (\ref{eq:CP}), we can solve the following optimization problem
\begin{equation}
\label{eq:coe_ten}
    \min \limits_{\{ \mat{U}^{(k)}\}_{k=1}^d} h(\ten{X})= \frac{1}{2} \sum \limits_{n=1}^N \left( y_n-\langle [\![\mat{U}^{(1)}, \mat{U}^{(2)}, \ldots, \mat{U}^{(d)}]\!], \ten{B}_n \rangle \right )^2,
\end{equation}
where $y_n=y(\vecpar_n)$ and $\ten{B}_n=\ten{B}(\vecpar_n)$.


% We denote the $i$-th term of the univariate gPC expansion toward the $j$-th dimension $\uniGPC_{i}(\parm^{(j)})$ as $\uniGPC^{(j)}_{i}$.
% Given a $d$-dim problem, if we do $p$-order expansion over each dimension, the multivariate basis $\ten{B}(\vecpar)=\{\ten{B}_{i_1 \ldots i_d}(\vecpar) = \uniGPC^{(1)}_{i_1} \ldots \uniGPC^{(d)}_{i_d}, \{i_j = 0,1,\ldots,p\}_{j=1}^d \}$ will be a rank-1 tensor, which can be exactly represented as: 
% \begin{equation}
%   \ten{B(\vecpar)} =  \vect{\uniGPC}^{(1)} \circ \vect{\uniGPC}^{(2)} \circ \cdots \circ \vect{\uniGPC}^{(d)},
% \end{equation}
% The corresponding coefficient tensor $\ten{X}$ is unknown to us with $(p+1)^d$ variables in total, which seems to greatly increase the complexity compared to $\frac{(d+p)!}{d!p!}$. 

% However, the key ingredient here is to do a rank-$R$ tensor approximation towards the coefficient tensor:
% \begin{equation}\label{eq:coe_ten}
%     \ten{X} \approx \sum_{r=1}^R \mat{x}_r^{(1)} \circ \mat{x}_r^{(2)} \circ \cdots \circ \mat{x}_r^{(d)} = [\![\mat{U}^{(1)}, \mat{U}^{(2)}, \ldots, \mat{U}^{(d)}]\!].
% \end{equation}
% It decreases the number of unknown variables to $(p+1)dr$ which is only linear on $d$ and therefore effectively overcome the curse of dimensionality. 

\subsection{Automatic Rank Determination}
The low-rank tensor regression~\reff{eq:coe_ten} requires the rank of $\ten{X}$ to be determined {\it a-priori}, which is often infeasible in practice. In order to address this issue, we first choose a sufficiently large $R$ such that it is above the actual rank, then we choose a proper rank-shrinking penalty function to regularize~\reff{eq:coe_ten}.
%Some researchers adopted a greedy strategy to increase the rank parameter adaptively until convergence.

Specifically, we employ a group $\ell_{q}/ \ell_{2}$-norm regularization function to shrink the rank of $\ten{X}$: 
% \begin{equation}
% \label{eq:rank_penalty}
%     g(\ten{X}) = \{\sum \limits_{r=1}^R {\left[ \left( \sum \limits_{k=1}^d \| \mat{u}_{r}^{(k)} \|_2^2 \right)^{\frac{1}{2}} \right ]}^{q}\}^{\frac{1}{q}}, \quad q \in \left( 0, 1\right].
% \end{equation}
\begin{equation}
\label{eq:rank_penalty}
   g(\ten{X}) = \|\mat{v}\|_q, 
   \mat{v}= \left( \sum \limits_{k=1}^d \| \mat{u}_{r}^{(k)} \|_2^2 \right)^{\frac{1}{2}} , \quad q \in \left( 0, 1\right].
\end{equation}
This function puts $\mat{u}_r^{(k)}$, the $r$-th column of each $\mat{U}^{(k)}$, in the same group, and measures the $\ell_{q}/ \ell_{2}$ norm of all groups. As a result, one can shrink some groups to zero by reducing $g(\ten{X})$, leading to an automatic rank reduction. A smaller $q$ leads to a stronger shrinkage, and $q=1$ corresponds to a group lasso. 

By adding the penalty term \reff{eq:rank_penalty}, we have the following improved tensor regression model:
\begin{equation}
\label{eq:tensor_regression}
\begin{aligned}
        \min \limits_{\{\mat{U}^{(k)}\}_{k=1}^d} f(\ten{X}) = & h(\ten{X}) + \lambda g(\ten{X}).
\end{aligned}
\end{equation}
After solving this optimization problem, each obtained factor matrix $\mat{U}^{(k)}$ has a few common columns whose values are close to zero. These columns can be deleted and the actual rank of our obtained tensor becomes $\hat{R}\leq R$, where $\hat{R}$ is the number of remaining columns that are not deleted.
% \begin{equation}
% \label{eq:tensor_regression}
% \begin{aligned}
%         \min \limits_{\{\mat{U}^{(j)}\}_{j=1}^d} f(\ten{X}) = & h(\ten{X}) + \lambda g(\ten{X})\\
%         = & \frac{1}{2}\sum \limits_{n=1}^N \left[ {y}_n - \langle [\![\mat{U}^{(1)}, \mat{U}^{(2)}, \ldots, \mat{U}^{(d)}]\!], \ten{B}_n \rangle \right]^2 \\
%         + & \lambda \sum \limits_{r=1}^R {\left[ \left( \sum \limits_{j=1}^d \| \mat{u}_{r}^{(j)} \|_2^2 \right)^{\frac{1}{2}} \right ]}^{\frac{1}{q}},
% \end{aligned}
% \end{equation}

%\zz{(It's very unclear here. In the tensor regression you are trying to minimize $f(\ten{X})$, but here you are talking about how to minimize $L(\ten{X})$).}
It is non-trivial to minimize $f(\ten{X})$
since the regularization function $g(\ten{X})$ is usually non-differentiable and non-convex with respect to $\mat{U}^{(k)}$'s. 
Instead, we solve the following optimization problem in practice:
\begin{equation}
    \label{eq:tensor_regression_bound}
\begin{aligned}
        \min \limits_{\{\mat{U}^{(k)}\}_{k=1}^d} \hat{f}(\ten{X}) = & h(\ten{X}) + \lambda \hat{g}(\ten{X}).
\end{aligned}
\end{equation}
Here $\hat{g}(\ten{X})$ is a transformation of $g(\ten{X})$ obtained via the variational equality~\cite{jenatton2010structured}:
\begin{align}
\label{eq:subproblem_eta}
     \hat{g}(\ten{X}) = g(\ten{X}) = \min_{\boldsymbol{\eta} \in \R_{+}^R} \frac{1}{2}\sum \limits_{r=1}^R \frac{\sum \limits_{k=1}^d \| \mat{u}_{r}^{(k)} \|_2^2 }{{\eta}_r} + \frac{1}{2}\|\boldsymbol{\eta}\|_{\frac{q}{2-q}}.
\end{align}
Once $\{\mat{U}^{(k)}\}_{k=1}^d$ is given, the values of $\hat{g}(\ten{X})$ and $\hat{f}(\ten{X})$ can be estimated by setting the elements of $\boldsymbol{\eta}$ as
\begin{equation}
\label{eq:eta_solution}
    {\eta}_r = ({{z}_r})^{2-q}\| \mat{z} \|_{q}^{q-1}, \quad \forall \; r=1,\ldots,R,
\end{equation}
where ${z}_r = {\left( \sum \limits_{k=1}^d \| \mat{u}_{r}^{(k)} \|_2^2\right)}^{\frac{1}{2}}$.   
%\zz{The above solution seems to be the minimum of the upper bound of regularization function, not the upper bound of the cost function.} 
%Yes, it is only the minimum of a sub-problem

Problem~\reff{eq:tensor_regression_bound} can be solved via an alternating algorithm such as a block coordinate descent solver or alternating direction method of multipliers. Due to the page limitation, we omit the details in this paper and will explain the detailed optimization algorithm in an extended journal paper. 

% \subsection{A Block Coordinate Solver for  Eq.~\reff{eq:tensor_regression}}
% An alternating solver is proposed to decompose \reff{eq:tensor_regression} into sub-problems of $\{\mat{U}^{(j)}\}_{j=1}^d$ and $\vect{\eta}$ which have analytical solutions. 

% \textbf{$\mat{U}^{(j)}$-subproblem:} Suppose $\mat{U}^{(-j)}$ and $\vect{\eta}$ are fixed, we have
% \begin{equation}\label{eq:sub_Uj}
% \begin{aligned}
%     %\min_\limit{\mat{U}^{(j)}} 
%     f_j(\mat{U}^{(j)}) = & 
%     \frac{1}{2} \sum_\limit{i=1}^N \left[ y_i -
%     \langle \mat{U}^{(j)}, \mat{X}_{i_{(j)}} \mat{U}^{(-j)} \rangle 
%     \right]^2 + \frac{1}{2}\sum_\limit{r=1}^R \frac{ \| \mat{U}_{:,r}^{(j)} \|_2^2 }{{\eta}_r} \\
%     = & \frac{1}{2} \sum_\limit{i=1}^N \left[ y_i -
%     \langle \mat{U}^{(j)}, \tilde{\mat{X}}_i_{(j)} \rangle
%     \right]^2 + \frac{\lambda}{2}\Tr(\mat{U}^{(j)} \Lambda \mat{U}^{(j)}^T)
% \end{aligned}
% \end{equation}
% \begin{equation}
% \begin{aligned}
% \tilde{\mat{X}}_i_{(j)} = & \vect{\uniGPC}^{(j)}(\vecpar_i)[\vect{\uniGPC}^{(d)}(\vecpar_i)^T \mat{U}^{(d)} * \cdots \vect{\uniGPC}^{(j+1)}(\vecpar_i)^T \mat{U}^{(j+1)}  *\\ 
% &\vect{\uniGPC}^{(j-1)}(\vecpar_i)^T \mat{U}^{(j-1)} * 
% \cdots \vect{\uniGPC}^{(1)}(\vecpar_i)^T \mat{U}^{(1)}]
% \end{aligned}
% \end{equation}
% where $\mat{X}_{(j)}$ denotes the $j$-th dimension unfolding operator, $\mat{U}^{(-j)} = \mat{U}^{(M)} \odot \cdots \odot \mat{U}^{(j-1)} \odot \mat{U}^{(j+1)} \cdots \odot \mat{U}^{(1)}$ with $\odot$ denotes the Khatri-Rao product and $*$ denotes the Hadamard product.
% Take the derivative over $\mat{U}^{(j)}$ and make it zero, the analytical solution to minimizing Eq.~\reff{eq:sub_Uj} is as follows:
% \begin{equation}\label{eq:sol_sub_U}
%     \text{vec}(\mat{U}^{(j)}) = {(\mat{\Phi}^T\mat{\Phi} + \lambda \tilde{\mat{\Lambda}})}^{-1} \mat{\Phi}^T \vect{y},
% \end{equation}
% where $\mat{\Phi} = \{\vect{\Phi}_i = \text{vec}(\tilde{\ten{X}}_i_{(j)})^T, i=1,2,\ldots,N \}$ and $\mat{\tilde{\Lambda}} = \text{diag}(\frac{1}{{\eta}_1},\ldots,\frac{1}{{\eta}_{R}}) \circ \mat{I}$.

% \textbf{$\eta$-subproblem:} The subproblem and its analytical solution are shown as  Eqs.~\reff{eq:subproblem_eta} and~\reff{eq:eta_solution} respectively.

\subsection{Adaptive Sampling Strategy}
%\zz{Please provide more details for this section. For instance, what is the definition of Voronoi cell, and what is the key equation/criteria you will use to pick the samples?}
%The proposed tensor regression model effectively reduce the number of unknown variables, which in additionally reduce the number of needed samples.
%\zz{This section is still unclear. For instance, given that you have simulated $n$ samples, how do you move to the next sample? what is $\mat{a}$ in (13)? You talked about Tayler expansion, then what's the expansion order? The definition of (12) is also unclear. }
Another fundamental question is how to select the parameter samples $\{ \vecpar_n\}_{n=1}^N$ for simulation. The method in~\cite{zhang2016big} uses some Monte Carlo random samples. Instead, this paper reduces the simulation cost by selecting only a few informative samples for detailed device- or circuit-level simulations.

We first use the Latin Hybercube (LH) sampling to generate 
an initial sample set ${\Omega}$. Then we employ an exploration step via the Voronoi diagram to measure the sample density in $\Omega$.
%A Voronoi diagram can measure the sample density in $\Omega$.
%Given a set of existing samples $\Omega \subset \R^d$, 
Given two distinct samples $\vecpar_i, \vecpar_j \in \Omega$, a Voronoi cell $C_i(\vecpar_i)$ covers the region that are closest to $\vecpar_i$. It is defined as the intersection of a set of half-planes (hp):
\begin{equation}
\begin{split} %\bigcap_\limit{} error in local LATEX
         C_i(\vecpar_i) = &\bigcap_{\vecpar_j\in \Omega \setminus \vecpar_i} \hp(\vecpar_i,\vecpar_j)\\
         \hp(\vecpar_i,\vecpar_j)=&\{\vecpar \in \R^d | \; \|\vecpar-\vecpar_i\| \le \|\vecpar-\vecpar_j\|\}.
\end{split}
\end{equation}    
It is intractable to calculate an Voronoi cell exactly in a high-dimensional space. 
However, we can easily estimate it via Monte Carlo~\cite{crombecq2009space}. 
The sample density of $C_i$ is approximated by counting the number of samples that are closest to $\vecpar_i$. 
Each sample in $\Omega $ determines one Voronoi cell with itself as the center, and we can select a new sample from the cell region with the lowest density.

If the performance metric $y(\vecpar)$ is known to be highly nonlinear, we can further exploit its non-linearity. Given $\vecpar$ and a Voronoi cell center $\mat{a}$, we measure the nonlineary of $y(\vecpar)$ as
\begin{equation}
    \gamma(\vecpar) = |\hat{y}(\vecpar) - \hat{y}(\mat{a}) - \nabla \hat{y}(\mat{a})^T(\vecpar-\mat{a}) |.
\end{equation}
We select a new sample as the one with largest $\gamma(\vecpar)$ in a Voronoi cell with the lowest sample density.
%which is a good trade-off between exploration and exploitation. 
This method can be easily extended to a batch version by searching the top-$K$ least-sampled regions.


%Adaptive sampling scheme is very popular to reduce the number of needed samples. In our framework, we adopt the Latin Hybercube (LH) sampling as initialization. 
%To search for informative samples, firstly, lots of MC samples are used to estimate a Voronoi diagram~\cite{crombecq2009space}, and we can estimate a Voronoi cell with least sampling density. Then we do Taylor expansion on the samples~\cite{mo2017taylor} which fall on the selected cell to measure the nonlinearity of the surrogate. In other words, the selected sample will be the most nonlinear one in the least sampled cell region, which is a good trade-off between exploration and exploitation. The overall algorithm is summarized in Alg.~\reff{alg:adaptive_reg}.
% \begin{algorithm}[t]
%   \caption{Adaptive Tensor Regression}
%   \label{alg:adaptive_reg}
%   %\KwIn{Basis tensor $\ten{X}$, initial samples $\{\vecpar_i, y(\vecpar_i)\}_{i=1}^N$}
%   %\KwOut{Coefficient tensor $\ten{X}$}
%     \textbf{Step 1:} Solve regression problem~\reff{eq:tensor_regression}\\
%     \textbf{Step 2:} Shrink rank if possible. If not converge, go to the next step\\
%     \textbf{Step 3:} Select \& simulate new samples. Back to Step 1
% \end{algorithm}





%\subsection{Regularization parameter}
%Cross validation or LOO 


% \section{Sampling setting}
% \subsection{Initial sampling}

% \subsection{Sampling strategy}
% Statistical sampling is hard since we apply a pure optimization framework. 

% In this case, we want to develop a model-free sampling strategy. To make use of polynomial, the gradient information is easy to extract, trying to make use of the model information. 

% Exploration: Space-filling\\
% Exploitation: Nonlinearity measurement\\






==> EPEPS'20_Tensor_Regression_for_UQ/related_works.tex <==
\section{Related works}
\label{sec:related works}


==> motivation.tex <==
\section{Motivation}
\label{sec:motivation}


==> related_works.tex <==
\section{Related works}
\label{sec:related works}

